Multimodal LLMs for health grounded in individual-specific data

Foundation large language models (LLMs) have shown an impressive ability to solve tasks across a wide range of fields including health. To effectively solve personalized health tasks, LLMs need the ability to ingest a diversity of data modalities that are relevant to an individual's health status. In this paper, we take a step towards creating multimodal LLMs for health that are grounded in individual-specific data by developing a framework (HeLM: Health Large Language Model for Multimodal Understanding) that enables LLMs to use high-dimensional clinical modalities to estimate underlying disease risk. HeLM encodes complex data modalities by learning an encoder that maps them into the LLM's token embedding space and for simple modalities like tabular data by serializing the data into text. Using data from the UK Biobank, we show that HeLM can effectively use demographic and clinical features in addition to high-dimensional time-series data to estimate disease risk. For example, HeLM achieves an AUROC of 0.75 for asthma prediction when combining tabular and spirogram data modalities compared with 0.49 when only using tabular data. Overall, we find that HeLM outperforms or performs at parity with classical machine learning approaches across a selection of eight binary traits. Furthermore, we investigate the downstream uses of this model such as its generalizability to out-of-distribution traits and its ability to power conversations around individual health and wellness.

==> tables/individual_corrs.tex <==
\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_all_cause_mortality.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for All Cause Mortality.}}
\label{appendix:fig:corr_all_cause_mortality}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_diabetes.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for Diabetes.}}
\label{appendix:fig:corr_diabetes}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_hypertension.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for Hypertension.}}
\label{appendix:fig:corr_hypertension}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_major_depression.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for Major Depression.}}
\label{appendix:fig:corr_major_depression}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_migraine.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for Migraine.}}
\label{appendix:fig:corr_migraine}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_myocardial_infarction.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for Myocardial Infarction.}}
\label{appendix:fig:corr_myocardial_infarction}
\end{center}
\vskip -0.2in
\end{figure*}
\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/corr_stroke.pdf}
}
\caption{\textbf{Spearman's rank correlation between different methods' scores for Stroke.}}
\label{appendix:fig:corr_stroke}
\end{center}
\vskip -0.2in
\end{figure*}


==> tables/table_01_backup.tex <==
\begin{table*}[t]
\caption{Comparison of AUC and AUPRC for LLM-based classifiers vs. Logistic regression. The baseline approach uses age, sex and BMI as model features, while the expanded set also includes 11 additional clinical and wellness traits. The mean AUC/AUPRC along with standard errors in parenthesis were calculated across 1000 bootstrapped samples.}
\label{table:llm_logreg_perf}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{llllll}
\toprule
\textbf{Phenotype} & \textbf{Model} & \textbf{Baseline AUC} & \textbf{Expanded Set AUC} & \textbf{Baseline AUPRC} & \textbf{Expanded Set AUPRC} \\
\midrule
All Cause Mortality & Zero-shot & 0.56 (0.030) & 0.61 (0.031) & 0.08 (0.011) & 0.10 (0.016) \\
 & Few-shot & 0.63 (0.032) & 0.63 (0.029) & 0.11 (0.022) & 0.10 (0.014) \\
 & Soft Prompt & 0.71 (0.026) & 0.68 (0.025) & 0.13 (0.019) & 0.13 (0.019) \\
 & \textbf{Logistic Regression} & \textbf{0.70 (0.025)} & \textbf{0.70 (0.025)} & \textbf{0.16 (0.025)} & \textbf{0.14 (0.022)} \\
\midrule
Diabetes & Zero-shot & 0.71 (0.019) & 0.64 (0.021) & 0.25 (0.025) & 0.19 (0.022) \\
 & Few-shot & 0.72 (0.021) & 0.67 (0.021) & 0.23 (0.027) & 0.20 (0.024) \\
 & Soft Prompt & 0.73 (0.019) & 0.68 (0.029) & 0.28 (0.031) & 0.17 (0.027) \\
 & \textbf{Logistic Regression} & \textbf{0.75 (0.020)} & \textbf{0.79 (0.022)} & \textbf{0.28 (0.032)} & \textbf{0.38 (0.037)} \\
\midrule
Hypertension & Zero-shot & 0.70 (0.015) & 0.69 (0.013) & 0.66 (0.021) & 0.65 (0.018) \\
 & Few-shot & 0.72 (0.013) & 0.71 (0.014) & 0.67 (0.022) & 0.65 (0.023) \\
 & Soft Prompt & 0.71 (0.014) & 0.73 (0.013) & 0.65 (0.019) & 0.59 (0.024) \\
 & \textbf{Logistic Regression} & \textbf{0.73 (0.012)} & \textbf{0.77 (0.012)} & \textbf{0.68 (0.019)} & \textbf{0.73 (0.019)} \\
\midrule
Major Depression & Zero-shot & 0.52 (0.022) & 0.58 (0.023) & 0.16 (0.013) & 0.20 (0.021) \\
 & Few-shot & 0.53 (0.020) & 0.57 (0.021) & 0.16 (0.013) & 0.20 (0.019) \\
 & Soft Prompt & 0.60 (0.021) & 0.46 (0.020) & 0.23 (0.026) & 0.12 (0.010) \\
 & \textbf{Logistic Regression} & \textbf{0.60 (0.021)} & \textbf{0.63 (0.022)} & \textbf{0.23 (0.022)} & \textbf{0.23 (0.022)} \\
\midrule
Migraine & Zero-shot & 0.49 (0.028) & 0.45 (0.035) & 0.04 (0.008) & 0.04 (0.005) \\
 & Few-shot & 0.42 (0.041) & 0.42 (0.030) & 0.04 (0.009) & 0.03 (0.004) \\
 & Soft Prompt & 0.65 (0.034) & 0.52 (0.038) & 0.07 (0.016) & 0.04 (0.005) \\
 & \textbf{Logistic Regression} & \textbf{0.69 (0.036)} & \textbf{0.70 (0.035)} & \textbf{0.08 (0.015)} & \textbf{0.09 (0.020)} \\
\midrule
Myocardial Infarction & Zero-shot & 0.59 (0.029) & 0.61 (0.026) & 0.09 (0.012) & 0.09 (0.012) \\
 & Few-shot & 0.68 (0.030) & 0.62 (0.027) & 0.14 (0.025) & 0.10 (0.014) \\
 & Soft Prompt & 0.70 (0.026) & 0.68 (0.024) & 0.16 (0.026) & 0.13 (0.020) \\
 & \textbf{Logistic Regression} & \textbf{0.72 (0.028)} & \textbf{0.73 (0.026)} & \textbf{0.15 (0.024)} & \textbf{0.20 (0.031)} \\
\midrule
Stroke & Zero-shot & 0.52 (0.036) & 0.55 (0.029) & 0.05 (0.012) & 0.05 (0.007) \\
 & Few-shot & 0.58 (0.035) & 0.54 (0.031) & 0.05 (0.009) & 0.04 (0.005) \\
 & Soft Prompt & 0.58 (0.039) & 0.52 (0.032) & 0.07 (0.013) & 0.05 (0.006) \\
 & \textbf{Logistic Regression} & \textbf{0.62 (0.036)} & \textbf{0.64 (0.038)} & \textbf{0.07 (0.012)} & \textbf{0.08 (0.017)} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/table_02_backup.tex <==
\begin{table}[ht]
\caption{Correlation between PaLM-E LLM risk score and logistic regression risk scores. We can see that the two methods produce risk profiles that are highly correlated indicating that the LLM is learning something similar to logistic regression.}
\label{table:llm_logreg_corr}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{ll}
\toprule
\textbf{Phenotype} & \textbf{Correlation} \\
\midrule
All Cause Mortality & 0.93 \\
Diabetes & 0.88 \\
Hypertension & 0.94 \\
Major Depression & 0.90 \\
Migraine & 0.82 \\
Myocardial Infarction & 0.93 \\
Stroke & 0.92 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/unseen_traits_backup.tex <==
\begin{table}[t]
% Content for this table is generated using http://google3/experimental/genomics/medgen/ukb_llm/notebooks/figures_and_tables/table_unseen_traits.ipynb
\caption{\textbf{(internal: unseen train performance using 1.5k individuals and the longer input context)}}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{llll}
\toprule
\textbf{Phenotype} & \textbf{Model} & \textbf{AUC} & \textbf{AUPRC} \\
\midrule
Cataract & Zero-shot & 0.59 (0.55--0.63) & 0.18 (0.15--0.22) \\
(prev=13.93\%) & Few-shot & 0.64 (0.60--0.67) & 0.19 (0.16--0.23) \\
 & LogReg & \textbf{0.72 (0.68--0.75)} & \textbf{0.27 (0.22--0.33)} \\
 & PaLM-E & \textbf{0.72 (0.69--0.75)} & \textbf{0.25 (0.21--0.29)} \\
\midrule
GERD & Zero-shot & \textbf{0.60 (0.56--0.64)} & \textbf{0.23 (0.19--0.27)} \\
(prev=17.41\%) & Few-shot & \textbf{0.58 (0.54--0.62)} & 0.21 (0.18--0.25) \\
 & LogReg & \textbf{0.59 (0.56--0.63)} & \textbf{0.25 (0.21--0.30)} \\
 & PaLM-E & \textbf{0.61 (0.57--0.64)} & \textbf{0.25 (0.21--0.30)} \\
\midrule
Hay Fever & Zero-shot & 0.50 (0.46--0.53) & 0.24 (0.21--0.28) \\
Eczema & Few-shot & 0.49 (0.46--0.52) & 0.25 (0.21--0.28) \\
(prev=24.18\%) & LogReg & \textbf{0.59 (0.56--0.62)} & \textbf{0.30 (0.27--0.35)} \\
 & PaLM-E & 0.48 (0.45--0.51) & 0.23 (0.20--0.26) \\
\midrule
Osteoarthritis & Zero-shot & 0.60 (0.56--0.63) & 0.35 (0.31--0.39) \\
(prev=27.60\%) & Few-shot & \textbf{0.63 (0.59--0.66)} & 0.36 (0.32--0.40) \\
 & LogReg & \textbf{0.66 (0.63--0.69)} & \textbf{0.42 (0.37--0.46)} \\
 & PaLM-E & \textbf{0.65 (0.63--0.68)} & \textbf{0.40 (0.36--0.44)} \\
\midrule
Pneumonia & Zero-shot & 0.56 (0.51--0.62) & 0.08 (0.06--0.11) \\
(prev=6.10\%) & Few-shot & 0.58 (0.52--0.63) & 0.08 (0.06--0.11) \\
 & LogReg & \textbf{0.69 (0.63--0.75)} & \textbf{0.18 (0.12--0.26)} \\
 & PaLM-E & \textbf{0.68 (0.63--0.74)} & 0.15 (0.10--0.22) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[t]
% Content for this table is generated using http://google3/experimental/genomics/medgen/ukb_llm/notebooks/figures_and_tables/table_unseen_traits.ipynb
\caption{\textbf{(internal: unseen train performance using 3k individuals and the shorter input context)}}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{llll}
\toprule
\textbf{Phenotype} & \textbf{Model} & \textbf{AUC} & \textbf{AUPRC} \\
\midrule
Cataract & Zero-shot & 0.58 (0.55--0.61) & 0.17 (0.15--0.20) \\
(prev=13.51\%) & Few-shot & 0.63 (0.60--0.65) & 0.18 (0.16--0.20) \\
 & PaLM-E & 0.51 (0.48--0.54) & 0.13 (0.12--0.15) \\
 & LogReg & \textbf{0.72 (0.69--0.74)} & \textbf{0.27 (0.23--0.31)} \\
\midrule
GERD & Zero-shot & 0.58 (0.55--0.60) & 0.22 (0.19--0.25) \\
(prev=17.33\%) & Few-shot & 0.57 (0.54--0.60) & 0.21 (0.18--0.23) \\
 & PaLM-E & 0.51 (0.48--0.53) & 0.17 (0.16--0.19) \\
 & LogReg & \textbf{0.61 (0.59--0.64)} & \textbf{0.26 (0.23--0.29)} \\
\midrule
Hay Fever & Zero-shot & 0.48 (0.46--0.51) & 0.23 (0.21--0.24) \\
Eczema & Few-shot & 0.46 (0.44--0.49) & 0.23 (0.21--0.25) \\
(prev=23.84\%) & PaLM-E & 0.50 (0.47--0.53) & 0.24 (0.22--0.26) \\
 & LogReg & \textbf{0.57 (0.55--0.60)} & \textbf{0.28 (0.26--0.31)} \\
\midrule
Osteoarthritis & Zero-shot & 0.60 (0.58--0.62) & 0.36 (0.33--0.39) \\
(prev=28.13\%) & Few-shot & 0.63 (0.61--0.65) & 0.38 (0.35--0.40) \\
 & PaLM-E & 0.48 (0.46--0.51) & 0.26 (0.24--0.28) \\
 & LogReg & \textbf{0.67 (0.65--0.69)} & \textbf{0.44 (0.40--0.47)} \\
\midrule
Pneumonia & Zero-shot & 0.56 (0.52--0.60) & 0.08 (0.06--0.10) \\
(prev=6.50\%) & Few-shot & 0.59 (0.55--0.63) & 0.08 (0.07--0.10) \\
 & PaLM-E & 0.46 (0.43--0.50) & 0.06 (0.05--0.07) \\
 & LogReg & \textbf{0.67 (0.63--0.71)} & \textbf{0.16 (0.12--0.20)} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
